Comparative Study of State-of-the-Art Matrix-Product-State Methods for Lattice Models with Large Local Hilbert Spaces

Lattice models consisting of high-dimensional local degrees of freedom without global particle-number conservation constitute an important problem class in the field of strongly correlated quantum many-body systems. For instance, they are realized in electron-phonon models, cavities, atom-molecule resonance models, or superconductors. In general, these systems elude a complete analytical treatment and need to be studied using numerical methods where matrix-product states (MPS) provide a flexible and generic ansatz class. Typically, MPS algorithms scale at least quadratic in the dimension of the local Hilbert spaces. Hence, tailored methods, which truncate this dimension, are required to allow for efficient simulations. Here, we describe and compare three state-of-the-art MPS methods each of which exploits a different approach to tackle the computational complexity. We analyze the properties of these methods for the example of the Holstein model, performing high-precision calculations as well as a finite-size-scaling analysis of relevant ground-state obervables. The calculations are performed at different points in the phase diagram yielding a comprehensive picture of the different approaches.

==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_0p5/ediff.dmrg3s.nph.15.do.10 <==
# min energy is -36.1599995629829607 obtained from symmps: gnu
#  m \DeltaE Var E0
+2.000000000000000E+01 +8.223252111652719E-06 +7.031685302265892E-07 -3.615970221019020E+01
+2.500000000000000E+01 +2.871549363604665E-06 +2.565836892545144E-07 -3.615989572775923E+01
+3.000000000000000E+01 +8.224287301494857E-07 +8.017812648332659E-08 -3.615996982396044E+01
+3.500000000000000E+01 +3.535642871389509E-07 +3.577711728892595E-08 -3.615998677809849E+01
+4.000000000000000E+01 +1.720061321652677E-07 +1.855880600814487E-08 -3.615999334324130E+01
+4.500000000000000E+01 +6.633869109500237E-08 +7.361484598242778E-09 -3.615999716417592E+01
+5.000000000000000E+01 +3.394470488130648E-08 +3.825527015930100E-09 -3.615999833554245E+01
+6.000000000000000E+01 +9.234685497705626E-09 +1.057105214653753E-09 -3.615999922905674E+01
+7.000000000000000E+01 +3.028049627409997E-09 +3.610749003268402E-10 -3.615999945348869E+01
+8.000000000000000E+01 +1.089722622270719E-09 +1.315243490958428E-10 -3.615999952357859E+01
+9.000000000000000E+01 +4.880599425132509E-10 +6.068657098258465E-11 -3.615999954533471E+01
+1.000000000000000E+02 +2.062364070444224E-10 +2.634260466222829E-11 -3.615999955552545E+01
+1.200000000000000E+02 +4.589210090068111E-11 +6.198781599036975E-12 -3.615999956132350E+01
+1.400000000000000E+02 +1.348655716690936E-11 +1.943955437796818E-12 -3.615999956249529E+01
+1.600000000000000E+02 +4.656059271933987E-12 +7.426991389823399E-13 -3.615999956281460E+01
+1.800000000000000E+02 +1.777142859479679E-12 +3.390923252182683E-13 -3.615999956291870E+01
+1.940000000000000E+02 +1.099808556447121E-12 +2.502327466607319E-13 -3.615999956294319E+01


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_0p5/ediff.dmrg3s.nph.15.do.5 <==
# min energy is -36.1599995629829607 obtained from symmps: gnu
#  m \DeltaE Var E0
+2.000000000000000E+01 +8.223252142306665E-06 +7.031656148541554E-07 -3.615970221018909E+01
+2.500000000000000E+01 +2.871549345919696E-06 +2.565752501544784E-07 -3.615989572775987E+01
+3.000000000000000E+01 +8.224287026395344E-07 +8.017625973352795E-08 -3.615996982396143E+01
+3.500000000000000E+01 +3.535642274030564E-07 +3.577713554775210E-08 -3.615998677810065E+01
+4.000000000000000E+01 +1.720060219289625E-07 +1.855801496633664E-08 -3.615999334324528E+01
+4.500000000000000E+01 +6.640128900688098E-08 +7.364537126070742E-09 -3.615999716191238E+01
+5.000000000000000E+01 +3.364771982563069E-08 +3.794377816673713E-09 -3.615999834628143E+01
+6.000000000000000E+01 +9.234291515901860E-09 +1.057087477515581E-09 -3.615999922907098E+01
+7.000000000000000E+01 +3.027410807038904E-09 +3.609620434441233E-10 -3.615999945351179E+01
+8.000000000000000E+01 +1.088305270275427E-09 +1.312233394461221E-10 -3.615999952362984E+01
+9.000000000000000E+01 +4.879793776556229E-10 +6.067439843755520E-11 -3.615999954533763E+01
+1.000000000000000E+02 +2.061352097232556E-10 +2.635199491123284E-11 -3.615999955552911E+01
+1.200000000000000E+02 +4.568164977258483E-11 +6.162611751007908E-12 -3.615999956133111E+01
+1.400000000000000E+02 +1.343939725024913E-11 +1.926739981285152E-12 -3.615999956249699E+01
+1.600000000000000E+02 +4.621671832702569E-12 +7.343522509768687E-13 -3.615999956281584E+01
+1.800000000000000E+02 +1.788539839339234E-12 +3.389184317181641E-13 -3.615999956291829E+01
+1.970000000000000E+02 +1.082909586310538E-12 +2.432770066562558E-13 -3.615999956294380E+01


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_0p5/ediff.dmrg3s.nph.23.do.10 <==
# min energy is -36.1599995629829607 obtained from symmps: gnu
#  m \DeltaE Var E0
+2.000000000000000E+01 +8.223252136804674E-06 +7.031689025387315E-07 -3.615970221018929E+01
+2.500000000000000E+01 +2.871549349063690E-06 +2.565814750558536E-07 -3.615989572775975E+01
+3.000000000000000E+01 +8.224286806315733E-07 +8.017718328342263E-08 -3.615996982396223E+01
+3.500000000000000E+01 +3.535642659169884E-07 +3.577722945031132E-08 -3.615998677809926E+01
+4.000000000000000E+01 +1.720061087818090E-07 +1.855876149139266E-08 -3.615999334324214E+01
+4.500000000000000E+01 +6.633869640049300E-08 +7.361511377845425E-09 -3.615999716417573E+01
+5.000000000000000E+01 +3.394469702132037E-08 +3.825541101304506E-09 -3.615999833554273E+01
+6.000000000000000E+01 +9.234678816717433E-09 +1.057128516383184E-09 -3.615999922905698E+01
+7.000000000000000E+01 +3.028069670374577E-09 +3.610743786463512E-10 -3.615999945348796E+01
+8.000000000000000E+01 +1.094774824842599E-09 +1.320528114451671E-10 -3.615999952339590E+01
+9.000000000000000E+01 +4.879988311212453E-10 +6.067352897005616E-11 -3.615999954533692E+01
+1.000000000000000E+02 +2.062303155551871E-10 +2.635251659173841E-11 -3.615999955552567E+01
+1.200000000000000E+02 +4.584926397638140E-11 +6.193217007032371E-12 -3.615999956132505E+01
+1.400000000000000E+02 +1.347240919191129E-11 +1.935434656291080E-12 -3.615999956249580E+01
+1.600000000000000E+02 +4.688285214985144E-12 +7.399168429805807E-13 -3.615999956281343E+01
+1.800000000000000E+02 +1.754152400107816E-12 +3.345710942153427E-13 -3.615999956291953E+01
+1.950000000000000E+02 +1.100201555752623E-12 +2.524933621621841E-13 -3.615999956294318E+01


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_0p5/ediff.dmrg3s.nph.7.do.5 <==
# min energy is -36.1599995629829607 obtained from symmps: gnu
#  m \DeltaE Var E0
+2.000000000000000E+01 +8.223320311769696E-06 +7.031650696110398E-07 -3.615970220772408E+01
+2.500000000000000E+01 +2.871617549573668E-06 +2.565752672311381E-07 -3.615989572529362E+01
+3.000000000000000E+01 +8.224969414669446E-07 +8.017643694223833E-08 -3.615996982149392E+01
+3.500000000000000E+01 +3.536324754659503E-07 +3.577711642433700E-08 -3.615998677563280E+01
+4.000000000000000E+01 +1.720742695988570E-07 +1.855803392326776E-08 -3.615999334077745E+01
+4.500000000000000E+01 +6.646953864177201E-08 +7.364527910719265E-09 -3.615999715944447E+01
+5.000000000000000E+01 +3.371597063951964E-08 +3.794377817191652E-09 -3.615999834381348E+01
+6.000000000000000E+01 +9.302541543792197E-09 +1.057085912618343E-09 -3.615999922660306E+01
+7.000000000000000E+01 +3.095665157921602E-09 +3.609669125114311E-10 -3.615999945104371E+01
+8.000000000000000E+01 +1.156539578193545E-09 +1.312156881500073E-10 -3.615999952116249E+01
+9.000000000000000E+01 +5.562217420595037E-10 +6.067074668232994E-11 -3.615999954286998E+01
+1.000000000000000E+02 +2.743777706267891E-10 +2.634938651232640E-11 -3.615999955306146E+01
+1.200000000000000E+02 +1.139232281778546E-10 +6.160872816847491E-12 -3.615999955886350E+01
+1.400000000000000E+02 +8.168470914892115E-11 +1.925696620547295E-12 -3.615999956002924E+01
+1.600000000000000E+02 +7.287032422547135E-11 +7.355695055780623E-13 -3.615999956034797E+01


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_0p5/ediff.pseudo_site.nph.15 <==
# min energy is -36.1599995629829607 obtained from symmps: gnu
#  m \DeltaE E0 disc.wt.
+1.000000000000000E+02 +2.572698028700417E-07 -3.615999026010700E+01 +5.296000000000000E-12
+2.000000000000000E+02 +1.655622149077895E-08 -3.615999896431000E+01 +9.285000000000000E-15
+4.000000000000000E+02 +1.601634321433771E-08 -3.615999898383200E+01 +3.027000000000000E-16
+6.000000000000000E+02 +1.057314622291288E-08 -3.615999918065800E+01 +2.569000000000000E-16
+9.000000000000000E+02 +5.806368239138104E-12 -3.615999956277300E+01 +1.556000000000000E-16


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_0p5/ediff.pseudo_site.nph.7 <==
# min energy is -36.1599995629829607 obtained from symmps: gnu
#  m \DeltaE E0 disc.wt.
+1.000000000000000E+02 +3.626093506682515E-07 -3.615998645102900E+01 +9.368000000000000E-12
+2.000000000000000E+02 +8.149783797915498E-11 -3.615999956003600E+01 +4.920000000000000E-14
+3.000000000000000E+02 +6.797453537718119E-11 -3.615999956052500E+01 +1.475000000000000E-15
+4.500000000000000E+02 +6.783639612129727E-11 -3.615999956053000E+01 +1.652000000000000E-16
+6.000000000000000E+02 +6.783639612129727E-11 -3.615999956053000E+01 +1.578000000000000E-16


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_1p5/ediff.dmrg3s.nph.15.do.5 <==
# min energy is -70.8626288747086335 obtained from dmrg3s: nph = 63, do = 10
#  m \DeltaE Var E0
+2.000000000000000E+01 +4.821929363148298E-05 +1.957424215339664E-06 -7.085921192879943E+01
+2.500000000000000E+01 +2.002298002823450E-05 +8.948297887900550E-07 -7.086120999370593E+01
+3.000000000000000E+01 +9.856026252372180E-06 +4.417044827844523E-07 -7.086193045077813E+01
+3.500000000000000E+01 +4.329216460635837E-06 +2.128077725660014E-07 -7.086232209504927E+01
+4.000000000000000E+01 +2.483127282270352E-06 +1.276280145484866E-07 -7.086245291378158E+01
+4.500000000000000E+01 +1.441887459102202E-06 +7.587132377630806E-08 -7.086252669877274E+01
+5.000000000000000E+01 +9.361247642999060E-07 +5.031405085590437E-08 -7.086256253844688E+01
+6.000000000000000E+01 +3.871903881919174E-07 +2.234614726198843E-08 -7.086260143737985E+01
+7.000000000000000E+01 +1.685753006553842E-07 +1.036535573019846E-08 -7.086261692901967E+01
+8.000000000000000E+01 +7.934278393485959E-08 +4.875645065728162E-09 -7.086262325227038E+01
+9.000000000000000E+01 +3.992095136891331E-08 +2.473844965969051E-09 -7.086262604580507E+01
+1.000000000000000E+02 +2.277123164128361E-08 +1.399534689477052E-09 -7.086262726107930E+01
+1.200000000000000E+02 +9.232672188504417E-09 +5.573730192669997E-10 -7.086262822045721E+01
+1.400000000000000E+02 +4.492927341174818E-09 +2.442375426280383E-10 -7.086262855632799E+01
+1.600000000000000E+02 +2.585028634258902E-09 +1.125778386012353E-10 -7.086262869152671E+01
+1.800000000000000E+02 +1.814931760242572E-09 +5.826565946129939E-11 -7.086262874609780E+01
+2.000000000000000E+02 +1.483240536142320E-09 +3.390777853642584E-11 -7.086262876960231E+01
+2.200000000000000E+02 +1.334373417795945E-09 +2.264648097247099E-11 -7.086262878015143E+01
+2.400000000000000E+02 +1.261571659850765E-09 +1.715982234286456E-11 -7.086262878531035E+01
+2.600000000000000E+02 +1.221149033584692E-09 +1.418203359596333E-11 -7.086262878817480E+01


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_1p5/ediff.dmrg3s.nph.31.do.10 <==
# min energy is -70.8626288747086335 obtained from dmrg3s: nph = 63, do = 10
#  m \DeltaE Var E0
+2.000000000000000E+01 +4.790012386535068E-05 +1.936555326435312E-06 -7.085923454600811E+01
+2.500000000000000E+01 +1.997962097295133E-05 +8.876431578502465E-07 -7.086121306624257E+01
+3.000000000000000E+01 +9.849952659524189E-06 +4.431124256223891E-07 -7.086193088116889E+01
+3.500000000000000E+01 +4.336210036424457E-06 +2.124876227132799E-07 -7.086232159946610E+01
+4.000000000000000E+01 +2.452869660240922E-06 +1.264041751108591E-07 -7.086245505791622E+01
+4.500000000000000E+01 +1.444526931179104E-06 +7.582343291476588E-08 -7.086252651173281E+01
+5.000000000000000E+01 +9.359470906858492E-07 +5.033498450926361E-08 -7.086256255103730E+01
+6.000000000000000E+01 +3.864200169779625E-07 +2.241069851423861E-08 -7.086260149197038E+01
+7.000000000000000E+01 +1.673814803316860E-07 +1.035292581955834E-08 -7.086261701361691E+01
+8.000000000000000E+01 +7.792000788106370E-08 +4.854130384499865E-09 -7.086262335309203E+01
+9.000000000000000E+01 +3.875568425778059E-08 +2.465436115944424E-09 -7.086262612837896E+01
+1.000000000000000E+02 +2.166221665108718E-08 +1.393728894624179E-09 -7.086262733966701E+01
+1.200000000000000E+02 +8.065146184778325E-09 +5.469595415184018E-10 -7.086262830319117E+01
+1.400000000000000E+02 +3.321894879974016E-09 +2.343567387043181E-10 -7.086262863931043E+01
+1.600000000000000E+02 +1.424987017116375E-09 +1.033188189056145E-10 -7.086262877373031E+01
+1.800000000000000E+02 +6.491558768700268E-10 +4.863842358565456E-11 -7.086262882870774E+01
+2.000000000000000E+02 +3.165638230885399E-10 +2.426297411447613E-11 -7.086262885227609E+01
+2.200000000000000E+02 +1.665084999644898E-10 +1.294118260488618E-11 -7.086262886290940E+01
+2.400000000000000E+02 +9.396744517728113E-11 +7.425001480879758E-12 -7.086262886804985E+01
+2.600000000000000E+02 +5.498710899745913E-11 +4.523645248737535E-12 -7.086262887081210E+01
+2.800000000000000E+02 +3.291537802096311E-11 +2.837783222056813E-12 -7.086262887237616E+01
+3.000000000000000E+02 +2.001277765119746E-11 +1.830033295565620E-12 -7.086262887329048E+01
+3.500000000000000E+02 +5.692954806523373E-12 +6.822778527512130E-13 -7.086262887430522E+01
+4.000000000000000E+02 +1.225505383354387E-12 +3.247475948956715E-13 -7.086262887462179E+01


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_1p5/ediff.dmrg3s.nph.31.do.5 <==
# min energy is -70.8626288747086335 obtained from dmrg3s: nph = 63, do = 10
#  m \DeltaE Var E0
+2.000000000000000E+01 +4.790966660363688E-05 +1.942932280602679E-06 -7.085923386978459E+01
+2.500000000000000E+01 +2.001420628043824E-05 +8.915573536591033E-07 -7.086121061543676E+01
+3.000000000000000E+01 +9.864959088254374E-06 +4.432511653910007E-07 -7.086192981777390E+01
+3.500000000000000E+01 +4.319682099544274E-06 +2.124644247433661E-07 -7.086232277067916E+01
+4.000000000000000E+01 +2.469024195998761E-06 +1.270732641524672E-07 -7.086245391316335E+01
+4.500000000000000E+01 +1.440808032917731E-06 +7.587150871736414E-08 -7.086252677526372E+01
+5.000000000000000E+01 +9.350396243043756E-07 +5.031323697444294E-08 -7.086256261534275E+01
+6.000000000000000E+01 +3.861137320787701E-07 +2.234710696782122E-08 -7.086260151367453E+01
+7.000000000000000E+01 +1.674976223853168E-07 +1.036594235471310E-08 -7.086261700538678E+01
+8.000000000000000E+01 +7.826257163009669E-08 +4.875837947689231E-09 -7.086262332881707E+01
+9.000000000000000E+01 +3.886906265739594E-08 +2.475810833976567E-09 -7.086262612034467E+01
+1.000000000000000E+02 +2.169353351766799E-08 +1.399819225497709E-09 -7.086262733744782E+01
+1.200000000000000E+02 +8.150287223731162E-09 +5.573715691029131E-10 -7.086262829715785E+01
+1.400000000000000E+02 +3.411281570124856E-09 +2.443875091997413E-10 -7.086262863297625E+01
+1.600000000000000E+02 +1.503959017188056E-09 +1.127910162275090E-10 -7.086262876813414E+01
+1.800000000000000E+02 +7.323677124538788E-10 +5.818198204063412E-11 -7.086262882281113E+01
+2.000000000000000E+02 +3.968164772885304E-10 +3.346983106449005E-11 -7.086262884658917E+01
+2.200000000000000E+02 +2.534325479769579E-10 +2.282108029977375E-11 -7.086262885674974E+01
+2.400000000000000E+02 +1.777895266916759E-10 +1.708338979864536E-11 -7.086262886211000E+01
+2.600000000000000E+02 +1.381875137505385E-10 +1.411284584562308E-11 -7.086262886491630E+01
+2.800000000000000E+02 +1.163377815400993E-10 +1.242879501509274E-11 -7.086262886646463E+01
+3.000000000000000E+02 +1.060119310755407E-10 +1.169996940293754E-11 -7.086262886719635E+01


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_1p5/ediff.dmrg3s.nph.63.do.10 <==
# min energy is -70.8626288747086335 obtained from dmrg3s: nph = 63, do = 10
#  m \DeltaE Var E0
+2.000000000000000E+01 +4.809983375736155E-05 +1.946675373151348E-06 -7.085922039404015E+01
+2.500000000000000E+01 +1.997962098658811E-05 +8.876431147420631E-07 -7.086121306624160E+01
+3.000000000000000E+01 +9.752546251516009E-06 +4.392339936625295E-07 -7.086193778364303E+01
+3.500000000000000E+01 +4.361728580204478E-06 +2.125585363751336E-07 -7.086231979115500E+01
+4.000000000000000E+01 +2.451670485475441E-06 +1.267139460480475E-07 -7.086245514289290E+01
+4.500000000000000E+01 +1.445963318544777E-06 +7.573314235403355E-08 -7.086252640994662E+01
+5.000000000000000E+01 +9.377189959969002E-07 +5.026646444669037E-08 -7.086256242547543E+01
+6.000000000000000E+01 +3.891222898385877E-07 +2.258152759487952E-08 -7.086260130048022E+01
+7.000000000000000E+01 +1.673118689787718E-07 +1.033817959180297E-08 -7.086261701854976E+01
+8.000000000000000E+01 +7.799573934088180E-08 +4.868826438754409E-09 -7.086262334772550E+01
+9.000000000000000E+01 +3.880749640339575E-08 +2.465842911043598E-09 -7.086262612470742E+01
+1.000000000000000E+02 +2.170914763142155E-08 +1.396694910842504E-09 -7.086262733634136E+01
+1.200000000000000E+02 +8.066311728435345E-09 +5.470428565760415E-10 -7.086262830310858E+01
+1.400000000000000E+02 +3.320017416154843E-09 +2.340792633444406E-10 -7.086262863944347E+01
+1.600000000000000E+02 +1.424806730855593E-09 +1.032726333858147E-10 -7.086262877374308E+01
+1.800000000000000E+02 +6.491384298125318E-10 +4.862302841242258E-11 -7.086262882870898E+01
+2.000000000000000E+02 +3.167769980554039E-10 +2.425971396015752E-11 -7.086262885226098E+01
+2.200000000000000E+02 +1.668626551775489E-10 +1.296979951510757E-11 -7.086262886288431E+01
+2.400000000000000E+02 +9.403843665260555E-11 +7.435325302917894E-12 -7.086262886804482E+01
+2.600000000000000E+02 +5.496545058125846E-11 +4.522196291258563E-12 -7.086262887081364E+01
+2.800000000000000E+02 +3.292400127926523E-11 +2.841043376383963E-12 -7.086262887237555E+01
+3.000000000000000E+02 +2.003604039452410E-11 +1.831120013674711E-12 -7.086262887328883E+01
+3.500000000000000E+02 +5.683729925549015E-12 +6.741274669338911E-13 -7.086262887430587E+01
+4.000000000000000E+02 +1.196828035977578E-12 +3.193140043508287E-13 -7.086262887462382E+01
+4.400000000000000E+02 -0.000000000000000E+00 +2.242261698158706E-13 -7.086262887470863E+01


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_1p5/ediff.pseudo_site.nph.15 <==
# min energy is -70.8626288747267807 obtained from dmrg3s: nph = 31, do = 10
#  m \DeltaE E0 disc.wt.
+1.000000000000000E+02 +2.939901342516113E-07 -7.086260804181300E+01 +2.151000000000000E-09
+2.000000000000000E+02 +4.466469580375653E-09 -7.086262855822100E+01 +4.866000000000000E-11
+4.000000000000000E+02 +1.113503496412841E-09 -7.086262879582100E+01 +5.863000000000000E-13
+6.000000000000000E+02 +1.081455457744367E-09 -7.086262879809200E+01 +3.290000000000000E-14
+9.000000000000000E+02 +1.079790366728496E-09 -7.086262879821000E+01 +1.355000000000000E-15


==> data/holstein/L_51_N_25_t_1p0_w_1p0_g_1p5/ediff.pseudo_site.nph.31 <==
# min energy is -70.8626288747267807 obtained from dmrg3s: nph = 31, do = 10
#  m \DeltaE E0 disc.wt.
+1.000000000000000E+02 +4.064420590165857E-07 -7.086260007317399E+01 +1.376000000000000E-09
+2.000000000000000E+02 +1.217531436348018E-08 -7.086262801195200E+01 +3.272000000000000E-11
+4.000000000000000E+02 +7.340607989779107E-09 -7.086262835455200E+01 +2.528000000000000E-13
+6.000000000000000E+02 +7.253340615761702E-09 -7.086262836073600E+01 +9.335000000000000E-15


==> disc_weight_scaling.tex <==
\ifthenelse{\boolean{rebuildCurrentBlock}}%
{%
	\setboolean{removeData}{true}%
}%
{%
	\ifthenelse{\boolean{buildCurrentBlockInline}}%
	{%
		\setboolean{removeData}{true}%
	}{}%
}%
%
\ifthenelse{\boolean{removeData}}%
{%
	\immediate\write18{rm -f \dstdir/scaling.dat}%
}{}%
%
\foreach \L in \Ls%
{%
	\immediate\write18{echo "L: \L" 1>&2}%
	\pgfmathsetmacro{\N}{int(\L/2)}%
%	N=\N%
%
	\def\d{1em04}%
	\immediate\write18{echo "dw E0 convergence discweight" > \datadir/../gs_energies.dat}%%
%	\IfFileExists{\datadir/../gs_fit.dat}{\immediate\write18{rm -f \datadir/../gs_fit.dat}}{}%
%
	\foreach \d in \dws%
	{%
		\ifthenelse{\boolean{rebuildCurrentBlock}}%
		{%
			\IfFileExists{\datadir/log/sym-groundstate-search.output}%
			{%
				\setboolean{rebuildData}{true}%
			}%
			{%
				\setboolean{rebuildData}{false}%		
			}%
		}%
		{%
			\ifthenelse{\boolean{buildCurrentBlockInline}}%
			{%
				\IfFileExists{\datadir/log/sym-groundstate-search.output}%
				{%
					\setboolean{rebuildData}{true}%
				}%
				{%
					\setboolean{rebuildData}{false}%
				}%
			}%
			{%
				\setboolean{rebuildData}{false}%
			}%
		}%
%
		\ifthenelse{\boolean{rebuildData}}%
		{%
			\immediate\write18{rm -f \datadir/../.NoValidResultsDetected.tmp}%
			\immediate\write18%
			{%
				if [ \string$(grep '\string^energy' \datadir/log/sym-groundstate-search.output | wc -l) = 0 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi
			}%
			\IfFileExists{\datadir/.not_converged}%
			{%
				\immediate\write18{touch  \datadir/../.NoValidResultsDetected.tmp}%
			}{}%
			\IfFileExists{\datadir/../.NoValidResultsDetected.tmp}%
			{%
				\immediate\write18{rm -f \datadir/../.NoValidResultsDetected.tmp}%
			}%
			{%	
%				\immediate\write18%
%				{%
%					echo \d	\
%					\string$(grep -B3 'stage \stage c' \datadir/log/sym-groundstate-search.output | tail -n3 | head -n1 | tr -d , | awk '{print \string$2,\string"\string\t\string",\string$5}') \
%					\string$(grep -B\string$((\L+6)) 'stage \stage c' \datadir/log/sym-groundstate-search.output | tail -n \string$((\L+6)) | sed "s/e-gain /e-gain:/" | awk "{print \string\$12}" | LC_NUMERIC=en_US.UTF-8 sort -g | tail -n1 )	\
%					>>  \datadir/../gs_energies.dat
%				}%
				\immediate\write18%
				{%
					echo \d	\
					\string$(grep '\string^energy' \datadir/log/sym-groundstate-search.output | tail -n1 | tr -d , | awk '{print \string$2,\string"\string\t\string",\string$5}') \
					\string$(grep -B\string$((\L+4)) '\string^energy' \datadir/log/sym-groundstate-search.output | tail -n \string$((\L+4)) | sed "s/e-gain /e-gain:/" | awk "{print \string\$12}" | LC_NUMERIC=en_US.UTF-8 sort -g | tail -n1 )	\
					>>  \datadir/../gs_energies.dat
				}%
			}%
		}{}%
	}%
	%
	\IfFileExists{\datadir/../gs_energies.dat}%
	{
		\immediate\write18%
		{if [ \string$(cat \datadir/../gs_energies.dat | wc -l) = 1 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
	}%
	{
		\immediate\write18{touch  \datadir/../.NoValidResultsDetected.tmp}%	
	}%
	\IfFileExists{\datadir/../.NoValidResultsDetected.tmp}%
	{}%
	{%
		\IfFileExists{\datadir/log/sym-groundstate-search.output}%
		{%
			\ifthenelse{\boolean{rebuildCurrentBlock}}%
			{%
				\tikzset{external/remake next=true}%
				\IfFileExists{\datadir/../gs_fit.dat}{\immediate\write18{rm -f \datadir/../gs_fit.dat}}{}%
			}%
			{%
				\ifthenelse{\boolean{buildCurrentBlockInline}}%
				{%
					\tikzset{external/export next=false}%
					\IfFileExists{\datadir/../gs_fit.dat}{\immediate\write18{rm -f \datadir/../gs_fit.dat}}{}%
				}{}%
			}%
			\begin{tikzpicture}%
				\begin{axis}
				[
					opacity	= 0,
					width	=	0.85\textwidth,
					height	=	0.25\textheight,
					xmode	=	log,
					xlabel	=	{\small Discarded weight},
					ylabel	=	{$\nicefrac{E_0}{L}$},
					legend pos	=	north west,
					legend style=
					{
						font=\tiny,
					},
				]
				%	
				\addplot
				[
					color=blue,
					thick,
					only marks,
					mark=x,
					unbounded coords=jump,
					error bars/.cd, 
					y dir=both,
					y explicit,
				] 
					table
					[
						x expr = \thisrowno{3},
						y expr = \thisrowno{1}/(\L),
						y error expr = 2.0*sqrt(\thisrowno{3}/\L), 
					]
					{\datadir/../gs_energies.dat};
				\addlegendentry{DMRG results};
				
				\makeatletter
					\addplot
					[
						no markers, 
						color=blue,
						thick,
					] 
						gnuplot 
						[
							raw gnuplot
						] 
						{
							set fit quiet;
							set fit logfile '/dev/null';
							set print "\datadir/../gs_fit.dat" append;
							set fit errorvariables;
							f(x) = a+abs(b)*x;
							fit f(x) '\datadir/../gs_energies.dat' u ($4):($2) via a,b;
							fit f(x) '\datadir/../gs_energies.dat' u ($4):($2):(2.0*sqrt($4)) yerrors via a,b;
							print \L,\N,a,a_err,b,b_err;
						};
				\makeatother
				
				\IfFileExists{\datadir/../gs_fit.dat}%
				{
					\immediate\write18%
					{if [ \string$(cat \datadir/../gs_fit.dat | wc -l) = 0 ]; then touch  \datadir/../.NoValidFit.tmp; fi}%
				}%
				{
					\immediate\write18{touch  \datadir/../.NoValidResultsDetected.tmp}%	
				}%
				
				\IfFileExists{\datadir/../.NoValidFit.tmp}%
				{
					\immediate\write18{rm -f \datadir/../.NoValidFit.tmp}%	
					\immediate\write18{rm -f \datadir/../.NoValidResultsDetected.tmp}%	
				}
				{
					\pgfplotstableread[header=false]{\datadir/../gs_fit.dat}{\DataUZero}
					\pgfplotstablegetelem{0}{2}\of\DataUZero 
					\pgfmathsetmacro{\Ea}{\pgfplotsretval}
					\pgfplotstablegetelem{0}{3}\of\DataUZero 
					\edef\Eaerr{\pgfplotsretval}
					\pgfplotstablegetelem{0}{4}\of\DataUZero 
					\pgfmathsetmacro{\Eb}{\pgfplotsretval}
					
					\addplot
					[
						domain	=	\xmin:\xmax,
						color=blue,
						dashed,
					]
						{linearFct(\Eb, \Ea)/\L};
					\pgfmathparse{\Ea/\L}
					\edef\E{\pgfmathresult}
					\addlegendentry{fit to $E_0/L=\pgfmathprintnumber[std,precision=4]{\E} \pm \pgfmathprintnumber[sci,precision=2]{\Eaerr}$};
				}
				\end{axis}
			\end{tikzpicture}%
		}{}%
%
		\IfFileExists{\datadir/../gs_fit.dat}%
		{%
			\immediate\write18%
			{%
				grep -v "inf.0" \datadir/../gs_fit.dat | grep -v "NaN" >> \dstdir/scaling.dat
			}%
		}{}%
	}%
}%
\ifthenelse{\boolean{rebuildCurrentBlock}}%
{%
	\IfFileExists{\datadir/log/sym-groundstate-search.output}%
	{%
		\setboolean{rebuildData}{true}%
	}%
	{%
		\setboolean{rebuildData}{false}%		
	}%
}%
{%
	\ifthenelse{\boolean{buildCurrentBlockInline}}%
	{%
		\setboolean{rebuildData}{true}%
	}%
	{%
		\setboolean{rebuildData}{false}%
	}%
}%
\vspace{-0.24\textheight}%


==> finite_size_scaling.tex <==
\setboolean{removeData}{true}%
\def\dataroot{data/holstein/symmps_with_bath_sites/}%
\edef\datadir{\dataroot/t_\noexpand\t_w_\noexpand\w_g_\noexpand\g/finite_size_scaling/L_\noexpand\L_N_\noexpand\N/\noexpand\blas/m_\noexpand\m_d_\noexpand\d_nph_\noexpand\nph}%
\edef\dstdir{\dataroot/t_\noexpand\t_w_\noexpand\w_g_\noexpand\g/finite_size_scaling}%
%
\ifthenelse{\boolean{rebuildData}}%
{%
	%		\immediate\write18{bash -c "export t=\t; export w=\w; export g=\g; export nph=\nph; export dw=\dw; python3 data/holstein/build_finite_size_scaling_datatable.py --t-hop \string\${t/\string\p/\string\.} --omega \string\${w/\string\p/\string\.} --gamma \string\${g/\string\p/\string\.} --n-phonons \string\${nph/\string\p/\string\.} --disc-wt \string\${dw/\string\p/\string\.} --root-dir data/holstein --out-file data/holstein/finite_size_scaling/t_\t_w_\w_g_\g" >&2}%
}{}%
%	
\setboolean{rebuildCurrentBlock}{false}%
\setboolean{buildCurrentBlockInline}{true}%
%
\input{disc_weight_scaling}%
%
\ifthenelse{\boolean{removeData}}%
{%
	\immediate\write18{rm -f data/holstein/finite_size_scaling/t_\t_w_\w_g_\g*gs_energy_fit}%
	\immediate\write18{rm -f \dstdir/scaling_output.dat}%
	\setboolean{rebuildData}{true}%
}{}%
%
\setboolean{rebuildCurrentBlock}{false}%
\setboolean{buildCurrentBlockInline}{true}%
%
\begin{figure}[!t]
	\centering
	%
	\input{the_actual_finite_size_scaling_plot}%
	%
	\caption
	{
		\captionContent
	}
\end{figure}%
\setboolean{removeData}{false}%

==> finite_size_scaling_order_parameter.tex <==
\begin{figure}[!t]
	\centering
%
	\ifthenelse{\boolean{rebuildCurrentBlock}}%
	{%
		\setboolean{removeData}{true}%
		\setboolean{rebuildData}{true}%
		\tikzset{external/remake next=true}%
	}%
	{%
		\ifthenelse{\boolean{buildCurrentBlockInline}}%
		{%
			\setboolean{removeData}{true}%
			\setboolean{rebuildData}{true}%
			\tikzset{external/export next=false}%
		}{}%
	}%
	%
	\ifthenelse{\boolean{rebuildData}}%
	{%
%		\immediate\write18{bash -c "export t=\t; export w=\w; export g=\g; export nph=\nph; export dw=\dw; python3 data/holstein/build_finite_size_scaling_datatable.py --t-hop \string\${t/\string\p/\string\.} --omega \string\${w/\string\p/\string\.} --gamma \string\${g/\string\p/\string\.} --n-phonons \string\${nph/\string\p/\string\.} --disc-wt \string\${dw/\string\p/\string\.} --root-dir data/holstein --out-file data/holstein/finite_size_scaling/t_\t_w_\w_g_\g" >&2}%
	}{}%
%	
	\ifthenelse{\boolean{removeData}}%
	{%
		\immediate\write18{bash -c "rm -f data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.*order_parameter_fit"}%
	}{}%
	\tikzsetnextfilename{PPDMRG-finite-size-scaling-order_parameter_t_\t-w_\w-g_\g}
%	
	\begin{tikzpicture}
		\begin{axis}
		[
			width	= 0.95\textwidth,
			height	= 0.3\textheight,
			xmin	= 0,
			xmax	= 0.02,
			xlabel	= {$1/L$},
			ylabel	= {$x_{\rm ph}(L)$},
			legend style	= {font=\scriptsize, at={\legendPosition}, anchor=south west},
			legend columns	= 1,
		]
			
			\addplot
			[
				color	= colorC,
				mark	= x,
				only marks,
				thick,
				restrict expr to domain	= {1/x}{\xmax:\xmin},
			]
			table
			[
				x expr	= 1/\thisrowno{0},
				y expr	= \thisrowno{6},
			]
			{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.symmps.\dw.\blas};
			\addlegendentry{\gls{PP-2DMRG}}
			
			\ifthenelse{\boolean{rebuildData}}%
			{%
				\makeatletter
					\addplot
					[
						no markers, 
						color=blue,
						thick,
						forget plot,
					] %					
						gnuplot 
						[
							raw gnuplot
						] 
						{
							set fit quiet;
							set fit logfile '/dev/null';
							set print "data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.symmps.\dw.\blas_order_parameter_fit" append;
							set fit errorvariables;
							f(x) = a+b*x+c*x*x;
							fit [1.0/\xmin:1.0/\xmax]f(x) 'data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.symmps.\dw.\blas' u (1.0/$1):7 via a,b,c;
							print a,a_err,b,b_err,c,c_err;
						};
				\makeatother
			}{}%
%
			\pgfplotstableread[header=false]{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.symmps.\dw.\blas_order_parameter_fit}{\Data}
			\pgfplotstablegetelem{0}{0}\of\Data 
			\xdef\ppEapp{\pgfplotsretval}
			\pgfplotstablegetelem{0}{1}\of\Data 
			\xdef\ppEaerrpp{\pgfplotsretval}
			\pgfplotstablegetelem{0}{2}\of\Data 
			\xdef\ppEbpp{\pgfplotsretval}
			\pgfplotstablegetelem{0}{3}\of\Data 
			\xdef\ppEberrpp{\pgfplotsretval}
			\pgfplotstablegetelem{0}{4}\of\Data 
			\xdef\ppEcpp{\pgfplotsretval}
			\pgfplotstablegetelem{0}{5}\of\Data 
			\xdef\ppEcerrpp{\pgfplotsretval}
%
			\addplot
			[
				forget plot,
				mark	= none,
				color	= colorC,
				thick,
				domain	= 0:0.02,
				samples	= 100,
			]
			{quadFct(\ppEcpp,\ppEbpp,\ppEapp)};
%
			\addplot
			[
				color	= colorA,
				mark	= o,
				only marks,
				thick,
			]
			table
			[
				skip rows between index={0}{2},
				x expr	= 1/\thisrowno{0},
				y expr	= \thisrowno{3},
			]
			{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.ps};
			\addlegendentry{\gls{PS-DMRG}}
%			
			\ifthenelse{\boolean{rebuildData}}%
			{%
				\makeatletter
				\addplot
				[
				no markers, 
				color=blue,
				thick,
				forget plot,
				] %					
				gnuplot 
				[
				raw gnuplot
				] 
				{
					set fit quiet;
					set fit logfile '/dev/null';
					set print "data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.ps_order_parameter_fit" append;
					set fit errorvariables;
					f(x) = a+b*x+c*x*x;
					fit [1.0/\xmin:1.0/\xmax]f(x) 'data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.ps' u (1.0/$1):($4) via a,b,c;
					print a,a_err,b,b_err,c,c_err;
				};
				\makeatother
			}{}%
			%		%			
			\pgfplotstableread[header=false]{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.ps_order_parameter_fit}{\Data}
			\pgfplotstablegetelem{0}{0}\of\Data 
			\xdef\ppEaps{\pgfplotsretval}
			\pgfplotstablegetelem{0}{1}\of\Data 
			\xdef\ppEaerrps{\pgfplotsretval}
			\pgfplotstablegetelem{0}{2}\of\Data 
			\xdef\ppEbps{\pgfplotsretval}
			\pgfplotstablegetelem{0}{3}\of\Data 
			\xdef\ppEberrps{\pgfplotsretval}
			\pgfplotstablegetelem{0}{4}\of\Data 
			\xdef\ppEcps{\pgfplotsretval}
			\pgfplotstablegetelem{0}{5}\of\Data 
			\xdef\ppEcerrps{\pgfplotsretval}
			
			\addplot
			[
				forget plot,
				mark	= none,
				color	= colorA,
				thick,
				domain	= 0:0.02,
				samples	= 100,
			]
			{quadFct(\ppEcps,\ppEbps,\ppEaps)};
			
			\addplot
			[
				color	= colorB,
				mark	= square,
				only marks,
				thick,
			]
			table
			[
				x expr	= 1/\thisrowno{0},
				y expr	= \thisrowno{6},
			]
			{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.dmrg3s};
			\addlegendentry{\gls{DMRG3S+LBO}}
			
			
			\ifthenelse{\boolean{rebuildData}}%
			{%
				\makeatletter
					\addplot
					[
						no markers, 
						color=blue,
						thick,
						forget plot,
					] %					
						gnuplot 
						[
							raw gnuplot
						] 
						{
							set fit quiet;
							set fit logfile '/dev/null';
							set print "data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.dmrg3s_order_parameter_fit" append;
							set fit errorvariables;
							f(x) = a+b*x+c*x*x;
							fit [1.0/\xmin:1.0/\xmax]f(x) 'data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.dmrg3s' u (1.0/$1):($7) via a,b,c;
							print a,a_err,b,b_err,c,c_err;
						};
				\makeatother
			}{}%
			%		%			
			\pgfplotstableread[header=false]{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.dmrg3s_order_parameter_fit}{\Data}
			\pgfplotstablegetelem{0}{0}\of\Data 
			\xdef\ppEalbo{\pgfplotsretval}
			\pgfplotstablegetelem{0}{1}\of\Data 
			\xdef\ppEaerrlbo{\pgfplotsretval}
			\pgfplotstablegetelem{0}{2}\of\Data 
			\xdef\ppEblbo{\pgfplotsretval}
			\pgfplotstablegetelem{0}{3}\of\Data 
			\xdef\ppEberrlbo{\pgfplotsretval}
			\pgfplotstablegetelem{0}{4}\of\Data 
			\xdef\ppEclbo{\pgfplotsretval}
			\pgfplotstablegetelem{0}{5}\of\Data 
			\xdef\ppEcerrlbo{\pgfplotsretval}
			
			\addplot
			[
				forget plot,
				mark	= none,
				color	= colorB,
				thick,
				domain	= 0:0.02,
				samples	= 100,
			]
			{quadFct(\ppEclbo,\ppEblbo,\ppEalbo)};
		\end{axis}
	\end{tikzpicture}
	\caption
	{
		\label{fig:ppdmrg:finite-size-scaling:t-\t_w-\w_g-\g:order-parameter}
		%
		Finite size scaling for the \gls{CDW} order-parameter of the Holstein model.
		%
		The model is evaluated for parameters $\omega/t=\protect\ReplaceStr{\w}$, $\gamma/t=\protect\ReplaceStr{\g}$ at nearly half filling where we set $N_{\rm el}=\frac{L-1}{2}$.
	}
\end{figure}

==> the_actual_finite_size_scaling_plot.tex <==

\pgfplotstableread[header=false]{\dstdir/scaling.dat}{\DataCPU}
\pgfplotstablegetrowsof{\DataCPU}
\pgfmathtruncatemacro{\lastrowoftable}{int(\pgfplotsretval-1)}%
\pgfplotstablegetelem{\lastrowoftable}{0}\of\DataCPU
\xdef\Lmaxforfit{\pgfplotsretval}

\ifthenelse{\boolean{rebuildCurrentBlock}}%
{%
	\tikzset{external/remake next=true}%
}%
{%
	\ifthenelse{\boolean{buildCurrentBlockInline}}%
	{%
		\tikzset{external/export next=false}%
	}{}%
}%

\tikzsetnextfilename{PPDMRG-finite-size-scaling-t_\t-w_\w-g_\g}
%	
\pgfdeclareplotmark{xocgC}%
{%
	\pgfmathtruncatemacro{\ocgnumber}{int(\pgfplotspointmetatransformed)*2+1}%
	\pgfsetstrokecolor{colorC}%
	\pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}%
	\pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}%
	\pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}%
	\pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}%
	\node[actions ocg={ocg\ocgname\ocgnumber}{}{ocg\ocgname51 ocg\ocgname101 ocg\ocgname151 ocg\ocgname201 ocg\ocgname251 ocg\ocgname301 ocg\ocgname351 ocg\ocgname401 ocg\ocgname451 ocg\ocgname501 ocg\ocgname601 ocg\ocgname701 ocg\ocgname801 ocg\ocgname901 ocg\ocgname1001}, draw opacity=0] {\pgfusepathqstroke};%
}%
\tikzset{external/export next=false}%
\begin{tikzpicture}
\begin{axis}
[
width	= 0.95\textwidth,
height	= 0.3\textheight,
xmin	= 0,
xmax	= 0.02,
xlabel	= {$1/L$},
ylabel	= {$E_0/L$},
legend style	= {font=\scriptsize, at={(0.95,0.075)}, anchor=south east},
legend columns	= 1,
title	= {$t=\ReplaceStr{\t}$, $w=\ReplaceStr{\w}$, $g=\ReplaceStr{\g}$},%
point meta min = 0, 
point meta max = 2000, 
]
\addplot
[
color	= colorC,
scatter,
mark	= xocgC,
only marks,
thick,
point meta={\thisrowno{0}},
error bars/.cd, 
y dir=both,
y explicit,
] 
table
[
x expr = 1.0/\thisrowno{0}, 
y expr = \thisrowno{2}/\thisrowno{0},
y error expr = \thisrowno{3}/\thisrowno{0}, 
]
{\dstdir/scaling.dat};
\addlegendentry{\gls{PP-2DMRG}}
%	
\ifthenelse{\boolean{rebuildData}}%
{%
	\makeatletter
	\addplot
	[
	no markers, 
	color=blue,
	thick,
	forget plot,
	] %					
	gnuplot 
	[
	raw gnuplot
	] 
	{
		set fit quiet;
		set fit logfile '/dev/null';
		set print "\dstdir/scaling_output.dat" append;
		set fit errorvariables;
		f(x) = a+b*x;
		fit f(x) '\dstdir/scaling.dat' u (1.0/$1):($3/$1):($4/$1) yerrors via a,b;
		print a,a_err,b,b_err;
	};
	\makeatother
}{}%
%		%			
\pgfplotstableread[header=false]{\dstdir/scaling_output.dat}{\Data}
\pgfplotstablegetelem{0}{0}\of\Data 
\xdef\ppEapp{\pgfplotsretval}
\pgfplotstablegetelem{0}{1}\of\Data 
\xdef\ppEaerrpp{\pgfplotsretval}
\pgfplotstablegetelem{0}{2}\of\Data 
\xdef\ppEbpp{\pgfplotsretval}
\pgfplotstablegetelem{0}{3}\of\Data 
\xdef\ppEberrpp{\pgfplotsretval}
%			
%			
%			
\addplot
[
mark	= none,
color	= colorC,
thick,
domain	= \xminMain:0.02,
samples	= 100,
forget plot,
]
{linearFct(\ppEbpp, \ppEapp)};
%			
\addplot
[
color	= colorA,
mark	= o,
only marks,
thick,
]
table
[
x expr	= 1/\thisrowno{0},
y expr	= \thisrowno{1}/\thisrowno{0},
]
{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.ps};
\addlegendentry{\gls{PS-DMRG}}
% 			
\ifthenelse{\boolean{rebuildData}}%
{%
	\makeatletter
	\addplot
	[
	no markers, 
	color=blue,
	thick,
	forget plot,
	] %					
	gnuplot 
	[
	raw gnuplot
	] 
	{
		set fit quiet;
		set fit logfile '/dev/null';
		set print "data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.ps_gs_energy_fit" append;
		set fit errorvariables;
		f(x) = a+b*x;
		fit f(x) 'data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.ps' u (1.0/$1):($2/$1):($3) yerrors via a,b;
		print a,a_err,b,b_err;
	};
	\makeatother
}{}%
%		%			
\pgfplotstableread[header=false]{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.ps_gs_energy_fit}{\Data}
\pgfplotstablegetelem{0}{0}\of\Data 
\xdef\ppEaps{\pgfplotsretval}
\pgfplotstablegetelem{0}{1}\of\Data 
\xdef\ppEaerrps{\pgfplotsretval}
\pgfplotstablegetelem{0}{2}\of\Data 
\xdef\ppEbps{\pgfplotsretval}
\pgfplotstablegetelem{0}{3}\of\Data 
\xdef\ppEberrps{\pgfplotsretval}
% 			
\addplot
[
forget plot,
mark	= none,
color	= colorA,
thick,
domain	= 0:0.02,
samples	= 100,
]
{linearFct(\ppEbps,\ppEaps)};
% 			
\addplot
[
color	= colorB,
mark	= square,
only marks,
thick,
]
table
[
x expr	= 1/\thisrowno{0},
y expr	= \thisrowno{1}/\thisrowno{0},
]
{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.dmrg3s};
\addlegendentry{\gls{DMRG3S+LBO}}
% 			
% 			
\ifthenelse{\boolean{rebuildData}}%
{%
	\makeatletter
	\addplot
	[
	no markers, 
	color=blue,
	thick,
	forget plot,
	] %					
	gnuplot 
	[
	raw gnuplot
	] 
	{
		set fit quiet;
		set fit logfile '/dev/null';
		set print "data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.dmrg3s_gs_energy_fit" append;
		set fit errorvariables;
		f(x) = a+b*x;
		fit f(x) 'data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.dmrg3s' u (1.0/$1):($2/$1):($3) yerrors via a,b;
		print a,a_err,b,b_err;
	};
	\makeatother
}{}%
%		%			
\pgfplotstableread[header=false]{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.dmrg3s_gs_energy_fit}{\Data}
\pgfplotstablegetelem{0}{0}\of\Data 
\xdef\ppEalbo{\pgfplotsretval}
\pgfplotstablegetelem{0}{1}\of\Data 
\xdef\ppEaerrlbo{\pgfplotsretval}
\pgfplotstablegetelem{0}{2}\of\Data 
\xdef\ppEblbo{\pgfplotsretval}
\pgfplotstablegetelem{0}{3}\of\Data 
\xdef\ppEberrlbo{\pgfplotsretval}
% 			
% 			
\addplot
[
forget plot,
mark	= none,
color	= colorB,
thick,
domain	= 0:0.02,
samples	= 100,
]
{linearFct(\ppEblbo,\ppEalbo)};

\coordinate (inset_position) at (axis description cs:0.975,0.125);
\coordinate (inset_position_two) at (axis description cs:0.1,0.92);
\end{axis}
% 		
%\begin{axis}
%[
%	at={(inset_position)},
%anchor	= south east,
%width	= 0.4\textwidth,
%height	= 0.15\textheight,
%title	= {CPU time},
%xlabel	= {$L$},
%ylabel	= {$t$ [h]},
%%xmax	= \Lmaxforfit,
%ymode	= log,
%title style	= {font=\scriptsize,yshift=-5pt},
%ticklabel style	= {font=\scriptsize},
%xlabel style	= {font=\scriptsize,yshift=5pt},
%ylabel style	= {font=\scriptsize,yshift=0pt},
%]
%\addplot
%[
%color	= colorC,
%mark	= x,
%thick,
%restrict expr to domain = {x}{0:\Lmaxforfit},
%]
%table
%[
%x expr	= \thisrowno{0},
%y expr	= \thisrowno{7}/3600,
%]
%{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.symmps.\dw.\blas};
%
%\addplot
%[
%color	= colorA,
%mark	= o,
%thick,
%]
%table
%[
%x expr	= \thisrowno{0},
%y expr	= \thisrowno{4}*24+\thisrowno{5}+\thisrowno{6}/60+\thisrowno{7}/3600,
%]
%{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.ps};
%
%\addplot
%[
%color	= colorB,
%mark	= square,
%thick,
%]
%table
%[
%x expr	= \thisrowno{0},
%y expr	= \thisrowno{7}/3600,
%]
%{data/holstein/finite_size_scaling/t_\t_w_\w_g_\g.dmrg3s};
%
%\end{axis}

\foreach \L in \Ls
{
	\def\d{1em04}
	\pgfmathsetmacro{\N}{int(\L/2)}
	\IfFileExists{\datadir/../gs_energies.dat}%
	{
		\immediate\write18%
		{if [ \string$(cat \datadir/../gs_energies.dat | wc -l) = 1 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
		\IfFileExists{\datadir/../gs_fit.dat}%
		{
			\immediate\write18%
			{if [ \string$(cat \datadir/../gs_fit.dat | wc -l) = 0 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
			\immediate\write18%
			{if [ \string$(grep -v "NaN" \datadir/../gs_fit.dat | wc -l) = 0 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
			\immediate\write18%
			{if [ \string$(grep -v "inf" \datadir/../gs_fit.dat | wc -l) = 0 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
		}{}%
		
	}%
	{
		\immediate\write18{touch  \datadir/../.NoValidResultsDetected.tmp}%	
	}%
%
	\IfFileExists{\datadir/../.NoValidResultsDetected.tmp}%
	{	
		\immediate\write18{rm -f  \datadir/../.NoValidResultsDetected.tmp}%
	}%
	{
%
		\pgfplotstableread[header=false]{\datadir/../gs_fit.dat}{\DataUZero}%
		\pgfplotstablegetelem{0}{2}\of\DataUZero%
		\pgfmathsetmacro{\Ea}{\pgfplotsretval}%
		\pgfplotstablegetelem{0}{3}\of\DataUZero% 
		\edef\Eaerr{\pgfplotsretval}%
		\pgfplotstablegetelem{0}{4}\of\DataUZero%
		\pgfmathsetmacro{\Eb}{\pgfplotsretval}%
		%							
		\pgfmathparse{\eval{\Ea/\L}}%
		\edef\E{\pgfmathresult}%
		\pgfmathparse{\eval{\Eaerr}}%
		\edef\Eerr{\pgfmathresult}%
		\begin{axis}
		[
		y tick label style={
			/pgf/number format/.cd,
			fixed,
			fixed zerofill,
			precision=3,
			/tikz/.cd
		},
		name = ocgplot,
		ocg = {name=ocg\ocgname\L, ref=ocg\ocgname\L, status=invisible},
		inner sep=1pt,
		at	=	 {(inset_position_two)},
		anchor	= north west,
		width	=	0.395\textwidth,
		height	=	0.135\textheight,
		%			ymin	=	\E-0.00075,
		%			ymax	=	\E+0.0075,
		xmode	=	log,
		%			ymode	=	log,
		axis background/.style={fill=white, fill opacity=0.9},
		xlabel	=	{\tiny Discarded weight},
		ylabel	=	{\tiny $\nicefrac{E_0}{L}$},
		title	=	{\tiny $L=\L$, $E_0/L=\pgfmathprintnumber[std,precision=4]{\E} \pm \pgfmathprintnumber[sci,precision=1]{\Eerr}$},
		title style={yshift=-0.35em,xshift=-1em,fill=white, name=title},
		every tick label/.append style={font=\tiny,fill=white, fill opacity=0.9},
		xlabel style={name=xlabel,fill=white, fill opacity=0.9},
		]
		\addplot
		[
		color=blue,
		only marks,
		mark=x,
		forget plot,
		unbounded coords=jump,
		error bars/.cd, 
		y dir=both,
		y explicit,
		] 
		table
		[
		x expr = \thisrowno{3},
		y expr = \eval{(\thisrowno{1})/(\L)},
		y error expr = \eval{2.0*sqrt(\thisrowno{3}/\L)}, 
		%					y expr = \eval{(\thisrowno{1}-\Ea)/(\L)},
		%					y error expr = \eval{2.0*sqrt(\thisrowno{3}/\L)}, 
		]
		{\datadir/../gs_energies.dat};
		
		\addplot
		[
		domain	=	\xmin:\xmax,
		color=blue,
		dashed,
		]
		{linearFct(\Eb, \Ea)/\L};
		%				{linearFct(\Eb, 0)/\L};
		\end{axis}
	}%
}
\node[actions ocg={}{}{ocg\ocgname51 ocg\ocgname101 ocg\ocgname151 ocg\ocgname201 ocg\ocgname251 ocg\ocgname301 ocg\ocgname351 ocg\ocgname401 ocg\ocgname451 ocg\ocgname501 ocg\ocgname601 ocg\ocgname701 ocg\ocgname801 ocg\ocgname901 ocg\ocgname1001},fit = (title) (xlabel), inner sep = 0,yshift=-0.0575\textheight, inner xsep=2em, xshift=-0.0625\textwidth] {};
\end{tikzpicture}
